Multi-task Learning via Adaptation to Similar Tasks for Mortality Prediction of Diverse Rare Diseases

Mortality prediction of diverse rare diseases using electronic health record (EHR) data is a crucial task for intelligent healthcare. However, data insufficiency and the clinical diversity of rare diseases make it hard for directly training deep learning models on individual disease data or all the data from different diseases. Mortality prediction for these patients with different diseases can be viewed as a multi-task learning problem with insufficient data and large task number. But the tasks with little training data also make it hard to train task-specific modules in multi-task learning models. To address the challenges of data insufficiency and task diversity, we propose an initialization-sharing multi-task learning method (Ada-Sit) which learns the parameter initialization for fast adaptation to dynamically measured similar tasks. We use Ada-Sit to train long short-term memory networks (LSTM) based prediction models on longitudinal EHR data. And experimental results demonstrate that the proposed model is effective for mortality prediction of diverse rare diseases.

==> resources/discussion.tex <==
%\subsection{Discussion}



%In order to see if the learned embeddings of heterogeneous events are meaningful, we use LargeVIS~\autocite{tang2016visualizing} to get the 2D projection of all the heterogeneous events. 
%Notice that the same type of events with different attributes have distinct embedding vectors and will be plot in different positions in the pictures in Figure \ref{fig:embedding}.

\subsection{Case Study of Hierarchical Attention Mechanisms}
\begin{figure}[!ht]
\centering
\includegraphics[width=.9\linewidth]{resources/case.png}
\vspace{-.4cm}
\caption{Visualization of the event and temporal attention  }
\vspace{0.0cm}
\label{fig:temporal}
\end{figure}

To help experts to get some clinical insights by our hierarchical model, we visualize  the event attention and temporal attention mechanisms in Figure \ref{fig:temporal}.

From the colored frequency distribution histograms, we can see that irregular event sequences are adaptively segmented into groups. And we can see that some important events are picked out by the event attention score in the groups with high temporal attention scores. Taking the patient B as an example, although the events with the highest attention score of 19th and 24th group are lab tests for potassium and phenytoin with both normal results, resulting in the decreases of prediction score for death, the low temporal attention scores of these two groups indicate that these event groups will not influence the overall prediction result for the patient. Besides, we can see that there are many important events, such as unresponsive conscious level records and the drug input of levophed, in the event groups with high temporal attention score, which infers that the status of the patient is not well. So the final prediction of the model for the patient is death in hospital just as the truth. The subsequence consisting of critical events in the original long event sequence, captured by the hierarchical representations of clinical sequence, may provide long-range clinical insights for medical experts to evaluate the danger level and predict clinical endpoints of patients.

\subsection{Feature Analysis}
Important events for clinical prediction tasks can be picked out by the event attention mechanism in the hierarchical model.  The same events will get different event attention scores due to the local dependency with their surrounding events and the long-term dependency resulting from their phase in the temporal structure.  We divided the samples in each dataset into two groups according to the label to discover some differences of the statistics of the events between patients with different clinical endpoints. Thus, we calculated some statistics, including  the average event attention score,  the 1st quartile, the median, the 3rd quartile, the maximum of attention score and so on, of all kinds of events in each group. The top 10 events in each group  with highest median attention score and 3rd Quartile are listed in Table \ref{tab:top event}(for death prediction task) and Table \ref{tab:top event}(for ICU prediction task) respectively.  As the results, the top events in each group are similar both in term of median and the 1st quartile, indicating that these statistics can represent the distribution of attention score of critical events. We can find that important events in different dataset are different, which indicates that our model are able to capture critical information for different end point prediction tasks. 

\input{table_top_event}







==> table_events_statistics.tex <==
\begin{table}[!ht]

    \renewcommand\arraystretch{1}
    \centering
    \newcolumntype{e}{m{6cm}}
    \newcommand{\Multirow}[2]{\multirow{#1}{6cm}{#2}}
    \newcolumntype{a}{m{3cm}}
    \newcolumntype{n}{m{2cm}}
    \newcolumntype{v}{>{\centering\arraybackslash}m{2cm}}
    \newcommand{\twol}[2]{\makecell{#1 \\ #2}}
    \newcommand{\Chline}{\cmidrule{2-5}}
    
    \begin{tabular}{envvv}
        \toprule
            \textbf{event descriptions}    & 
            % \textbf{attribute list} & 
            \textbf{\twol{event name}{(top 2)}} & 
            \textbf{\twol{frequency}{(rank-in-all)}} &
            \textbf{\twol{coverage}{(rank-in-all)}}  & 
            \textbf{\twol{frequency}{per patient}} \\
        % \endfirsthead
        \midrule[\heavyrulewidth]
        \addlinespace
            \Multirow{2}{\textit{Chart events} include routine vital signs, ventilator settings, mental status, and so on.} 
            & Heart Rate & \twol{5171250}{(0.01\%)} & \twol{0.64}{(0.16\%)} & 173.4 \\ \Chline
            & SpO2 & \twol{3410702}{(0.01\%)} & \twol{0.479}{(0.33\%)} & 153.0 \\ % \Chline
            % & Respiratory Rate & \twol{3381160}{(0.02\%)} & \twol{0.479}{(0.33\%)} & 151.7 \\ % \Chline
            % & value(bigeminy, \newline fusion beats, \newline nodal bigeminy ...)  
            % & Ectopy Type & \twol{3242818}{(0.02\%)} & \twol{0.482}{(0.26\%)} & 144.6 \\
    
        \midrule[\heavyrulewidth]
        \addlinespace
            \Multirow{2}{\textit{Input events} are any fluid which have been administered to the patient: such as oral or tube feedings or intravenous solutions containing medications.}
            & 0.9\% Normal Saline & \twol{2363812}{(0.05\%)} & \twol{0.393}{(0.66\%)} & 129.2\\ \Chline
            & Propofol & \twol{369103}{(0.81\%)} & \twol{0.217}{(1.45\%)} & 36.5\\ % \Chline
            % & Dextrose 5\% & \twol{406345}{(0.74\%)} & \twol{0.298}{(1.04\%)} & 29.3\\ % \Chline
            % & duration, amount & Phenylephrine & \twol{93571}{(2.07\%)} & \twol{0.099}{(2.32\%)} & 20.3\\
        %\addlinespace[1cm]
        
        
        % \midrule[\heavyrulewidth]
        % \addlinespace
        %     \Multirow{3}{\textit{Datetime events} contain all date measurements about a patient in the ICU. For example, the dialysis.}
        %     & - & Equip Change [MM] & \twol{204762}{(1.24\%)} & \twol{0.037}{(4.02\%)} & 118.9\\ \Chline
        %     & - & INV\#1 Tubing Change [MM] & \twol{190605}{(1.32\%)} & \twol{0.155}{(1.92\%)} & 26.4\\ \Chline
        %     & - & Arterial line Insertion Date & \twol{182011}{(1.35\%)} & \twol{0.188}{(1.68\%)} & 20.8\\
    
        \midrule[\heavyrulewidth]
        \addlinespace
            \Multirow{2}{\textit{Lab events} contain all laboratory measurements for a given patient.} %including out patient data.
            & Hematocrit& \twol{881846}{(0.22\%)} & \twol{0.976}{(0.01\%)} & 19.4\\ \Chline
            & Potassium& \twol{845825}{(0.23\%)} & \twol{0.886}{(0.05\%)} & 20.5\\ % \Chline
            % & SODIUM & \twol{808489}{(0.24\%)} & \twol{0.886}{(0.05\%)} & 19.6\\ %\Chline
            % & value, flag(abnormal, delta, normal) & CREATININE & \twol{797476}{(0.25\%)} & \twol{0.846}{(0.07\%)} & 20.2\\ \Chline
            % & value, flag(abnormal, normal) & CHLORIDE & \twol{795568}{(0.25\%)} & \twol{0.886}{(0.05\%)} & 19.3\\
                
        \midrule[\heavyrulewidth]
        \addlinespace
            \Multirow{2}{\textit{Procedure events} contain procedures for patients.}
            & Chest X-Ray & \twol{32723}{(3.2\%)} & \twol{0.204}{(1.52\%)} & 3.44\\ \Chline
            & EKG & \twol{13962}{(4.35\%)} & \twol{0.167}{(1.82\%)} & 1.79\\ % \Chline
            % & Arterial Line & \twol{12703}{(4.46\%)} & \twol{0.189}{(1.66\%)} & 1.44\\
                
        \midrule[\heavyrulewidth]
        \addlinespace
            \Multirow{2}{\textit{Output events} are fluids which have either been excreted by the patient, such as urine output, or extracted from the patient.}
            & Chest Tubes CTICU CT 1 & \twol{151766}{(1.57\%)} & \twol{0.098}{(2.67\%)} & 33.2\\ \Chline
            & Urine & \twol{107465}{(1.93\%)} & \twol{0.075}{(3.05\%)} & 30.8\\ % \Chline
            % & Chest Tube \#1 & \twol{81128}{(2.23\%)} & \twol{0.071}{(3.1\%)} & 24.5\\
        \bottomrule
        \end{tabular}
\vspace{-8pt}
\caption{Statistics of High Frequency Examples in Different Types of Clinical Events}
\label{tab:clinical events}
\vspace{0.2cm}
\end{table}

==> table_top_event.tex <==
% table: top events in death according to median and 3rd
% \begin{table}[!ht]
% \renewcommand\arraystretch{1}
% \centering    
% \begin{tabular}{p{5cm}>{\centering\arraybackslash}p{2cm}p{5cm}>{\centering\arraybackslash}p{2cm}}
%     \toprule
%         \multicolumn{4}{c}{\textbf{death}} \\ 
%     \midrule
%         \multicolumn{2}{c}{sort by median} & \multicolumn{2}{c}{sort by 3rd Quartile} \\ 
%     \cmidrule(lr){1-2} \cmidrule(lr){3-4} 
%         event note & median & note & 3rd Quartile \\
%     \cmidrule(lr){1-2} \cmidrule(lr){3-4} 
%     % \endfirsthead
    
%         Blood\_Products & 0.996568 & Significant\_Events:defibrillation & 0.999906 \\ \addlinespace
%         Radiologic\_Study: thoracic lumbar sac & 0.989614 & Blood\_Products & 0.997947 \\ \addlinespace
%         INV\#2\_WaveformAppear:overshoot & 0.971317 & CORTISOL:abnormal & 0.99786 \\ \addlinespace
%         Pain\_Location: periumbilical & 0.96687 & Significant\_Events:resp arrest & 0.995923 \\ \addlinespace
%         Family\_Communication:family conference & 0.952387 & Radiologic\_Study: thoracic lumbar sac & 0.990783 \\ \addlinespace
%         Significant\_Events:resp arrest & 0.93346 & Family\_Communication:family conference & 0.985502 \\ \addlinespace
%         Erythromycin\_Oint.:held & 0.929935 & Restraint\_Location:left arm + right leg & 0.984022 \\ \addlinespace
%         Religion:ror & 0.925419 & IV\_Site\_Appear\_\#4:drainage & 0.982848 \\ \addlinespace
%         Education\_Topic\_\#2:hypertension & 0.889568 & Pain\_Location:right elbow & 0.979422 \\ \addlinespace

%     \midrule[\heavyrulewidth]

%         \multicolumn{4}{c}{\textbf{discharge}} \\ 
%     \midrule
%         \multicolumn{2}{c}{sort by median} & \multicolumn{2}{c}{sort by 3rd Quartile} \\ 
%     \cmidrule(lr){1-2} \cmidrule(lr){3-4} 
%         event note & median & note & 3rd Quartile \\
%     \cmidrule(lr){1-2} \cmidrule(lr){3-4} 

%         LENGTH\_OF\_URINE\_COLLECTION: normal; specimen received unlabeled & 0.999748 & Blood\_Products & 0.999889 \\ \addlinespace
%         Daily\_Wake\_Up: active isch/arth & 0.998826 & LENGTH\_OF\_URINE\_COLLECTION: normal;specimen received unlabeled & 0.999748 \\ \addlinespace
%         Significant\_Events:defibrillation & 0.99626 & Religion:prot & 0.999664 \\ \addlinespace
%         Ectopy\_Type: nodal trigeminy & 0.991996 & CBC: recent & 0.999629 \\ \addlinespace
%         RED\_TOP\_HOLD: normal & 0.988598 & Daily\_Wake\_Up: active isch/arth & 0.998826 \\ \addlinespace
%         Heart\_Rhythm: zoll paced & 0.970234 & Religion:catholic & 0.996502 \\ \addlinespace
%         Sx\_Equip\_Functioning:comment & 0.968053 & Significant\_Events:defibrillation & 0.996411 \\ \addlinespace
%         GI\#1\_Tube\_[Drain]: fecal & 0.967385 & Ectopy\_Type: nodal trigeminy & 0.991997 \\ \addlinespace
%         Family\_Communication: family conference & 0.960041 & RED\_TOP\_HOLD: normal & 0.988598 \\ \addlinespace
%         Blood\_Cultures: seny & 0.949292 & Radiologic\_Study:CT scan & 0.986526 \\ \addlinespace

%     \bottomrule
%     \addlinespace
%     \addlinespace
% \end{tabular}
% \caption{top event}
% \label{tab:top event}
% \end{table}



% top events in death and ICU according to median 

%\vspace{0.2cm}
\begin{table}[t]
\renewcommand\arraystretch{1}
\centering    
\begin{tabular}{p{6cm}>{\centering\arraybackslash}p{2cm}p{4cm}@{\hskip 1cm}>{\centering\arraybackslash}p{2cm}}
    \toprule
        \multicolumn{4}{c}{\textbf{Top Events (Sorted by Median of Event Attention Scores)}} \\ 
    \midrule
        \multicolumn{2}{c}{Death} & \multicolumn{2}{c}{ICU admission} \\
        event & attn score & event & atten score \\
    \cmidrule(lr){1-2} \cmidrule(lr){3-4}
    Blood Products & 0.9965 & Blood PH & 0.9998  \\
    Radiologic Study: thoracic lumbar sac & 0.9896 & Vancomycin & 0.9995\\
    NV\#2 Waveform Appear: overshoot & 0.9713 & Hematocrit (35-51) & 0.9967 \\
    Heart Rhythm & 0.9702 & Edimentation rate & 0.9885\\
    Pain Location: periumbilical & 0.9668 & Daily Weight & 0.9850 \\
    Family Communication & 0.9523 & Bilirubin Total & 0.9834 \\
     
    \bottomrule
\end{tabular}
\vspace{-4pt}
\caption{Top important events on the death prediction task and the ICU-admission prediction task.}
\label{tab:top event}
\end{table}
\vspace{0.3cm}
